Your decision path does matter in pre-training industrial recommenders with multi-source behaviors

Online service platforms offering a wide range of services through miniapps have become crucial for users who visit these platforms with clear intentions to find services they are interested in. Aiming at effective content delivery, cross-domain recommendation are introduced to learn high-quality representations by transferring behaviors from data-rich scenarios. However, these methods overlook the impact of the decision path that users take when conduct behaviors, that is, users ultimately exhibit different behaviors based on various intents. To this end, we propose HIER, a novel Hierarchical decIsion path Enhanced Representation learning for cross-domain recommendation. With the help of graph neural networks for high-order topological information of the knowledge graph between multi-source behaviors, we further adaptively learn decision paths through well-designed exemplar-level and information bottleneck based contrastive learning. Extensive experiments in online and offline environments show the superiority of HIER.

==> sec-rel.tex <==
\section{Related work}

\paratitle{Graph based Recommendation}
Graph based recommenders adeptly capture a variety of auxiliary contexts such as social networks~\cite{fan2019graph,yu2021self}, knowledge graphs~\cite{huang2021knowledge}, and heterogeneous graphs~\cite{lu2020meta} to enhance recommendations. 
Generally, information propagation is leveraged to explicitly represent complex relationships within the graph~\cite{wu2022graph} or to distinguish between different user interests for more robust recommendations~\cite{disengnn2022}. 
While these methods often perform well, their effectiveness is limited when target domain data is lacking or when linking items across domains, particularly with new items in the target domain, posing challenges for practical recommendation scenarios when target domain data is unavailable.



% \subsection{Cross-domain Recommendation}
\paratitle{Cross-domain Recommendation}
Cross-domain recommendation\cite{cdrsurvey2021,cdrsurvey2022} addresses cold-start issue of data-sparser target domains by leveraging the rich interactions in source domains.
A series of studies propose to learn a shared mapping matrix, and then perform alignment and transformation between source and target users/items~\cite{emcdr2017,ddtcdr2020}.
Recently, research focuses on bridging user preference in different domains~\cite{persontrans2022,lu2023three,li2023one}. 
However, most of the current approaches commonly involve interactions of target domains during training, which ignore a practical fact in real-world service platforms that items are completely non-overlapping across different domains and items in target domains are totally unavailable in the training stage.

\paratitle{Pre-training for Recommendation} 
Pre-training based recommenders often pre-train a recommender based on various auxiliary tasks, including sequence-level masking~\cite{gu2021self}, item-level~\cite{yao2021self} and graph-level~\cite{simgcl2022} contrastive learning.
In terms of the pre-training for cross-domain recommendation, several works have attempted to learn transferable interest based on sequence~\cite{peterrec2020}, collaborative graph~\cite{wang2021pre} and  knowledge graph~\cite{gao2023leveraging}. 
However, existing methods cannot handle the large gap between source and target domains, coupled with multiplex behaviors across domains. Although knowledge graphs are introduced to connect isolated items, they often aggregating auxiliary information indistinguishabily and overlook the impact of the decision path that users take when conduct behaviors thus fail to tackle the intricate situation in real-world service platforms. 

 


==> tab/data_tab.tex <==
\begin{table}[t]
    \centering
    \caption{Statistics of the source and target domains. }
    \label{tab:data_sta}
    \footnotesize
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{ c| c |c |c |c}
    \toprule
    \multirow{4}[5]{*}{\centering Source domains} & Datasets & \# Users & \# Entities & \# Interactions\\
    %\midrule
    \cmidrule{2-5}
    {} & Payment & 492,378,508 & 5,621,113 & 5,965,308,795  \\
    \cmidrule{2-5}	
    {} & Homepage Feed & 206,083,444 & 22,798 & 1,001,036,899  \\
    \cmidrule{2-5}	
    {} & Search & 27,029,750 & 146,776 & 51,007,668   \\
    \midrule
     \multirow{5}[5]{*}{\centering Target domains} & Datasets & \# Users & \# Items & \# Interactions\\
     \cmidrule{2-5}
     {} & Exercise & 1,363,747 & 344	 & 17,084,689	  \\
    \cmidrule{2-5}
    {} & Leasing & 137,949 & 2,464 & 1,387,138  \\
    \cmidrule{2-5}		
    % {} & Rental  & 222,692 & 9,220 & 2,076,059  \\
    % \cmidrule{2-5}		
    {} & E-governance & 105,070 & 12,749 & 1,023,478  \\
    \cmidrule{2-5}		
    {} & E-mall & 134,776 & 124,467 & 13,705,639  \\
    % \cmidrule{2-5}				
    % {} & Dining& 133,643 & 6,221 & 7,341,806  \\
    \midrule
    \multicolumn{2}{c|}{\centering \multirow{2}{*}{\centering Entity graph}}  & \# Entities & \# Relations & \# Triplets\\
    \cmidrule{3-5}
     \multicolumn{2}{c|}{} & {22,824,162} & {108} & {179,655,510} \\
    \bottomrule
    \end{tabular}        
\end{table}

==> tab/main_table_zero_shot.tex <==
\begin{table*}[t]\centering
\setlength{\tabcolsep}{1.5mm}{

\caption{Overall performance evaluation on six target domains. The best results are highlighted in boldface. } 
\label{tab:overall_result2}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c}

\toprule
\multirow{2}{*}{Tasks} & \multirow{2}{*}{Methods}
 & \multicolumn{2}{c|}{E-governance} 
& \multicolumn{2}{c|}{Digital Art} 
& \multicolumn{2}{c|}{Rental}  
& \multicolumn{2}{c|}{Food Delivery} 
& \multicolumn{2}{c|}{Daily Necessity} 
& \multicolumn{2}{c}{Dining} \\ 
% \cline{4-11}
%\midrule
\cmidrule{3-14}
%\midrule
 {} & {} 
 & {Hit} & {NDCG} & {Hit} & {NDCG} 
 & {Hit} & {NDCG} & {Hit} & {NDCG} 
 & {Hit} & {NDCG} & {Hit} & {NDCG}  \\
%  {Metrics} 
%  & {Hit@5} & {Hit@10} & {NDCG@5} & {NDCG@10} 
%  & {Hit@5} & {Hit@10} & {NDCG@5} & {NDCG@10} 
%  & {Hit@5} & {Hit@10} & {NDCG@5} & {NDCG@10} \\
%  \midrule
%   {Domains}
% & \multicolumn{4}{c|}{Target 1.} 
% & \multicolumn{4}{c|}{Target 2.} 
% & \multicolumn{4}{c}{Target 3.} \\  
\midrule
% {w/o pretrain}  	
&{DeepFM} 
& {0.2402} & {0.0406} 
& {0.2572} & {0.0480} 
& {0.0679} & {0.0092} 
& {0.1026} & {0.0136}
& {0.2195} & {0.0399} 
& {0.1604} & {0.0194} \\
% \midrule
\cmidrule{2-14} 
{} &{GRU4Rec} 
& {0.2376} & {0.0417} 
& {0.2428} & {0.0437} 
& {0.0666} & {0.0091} 
& {0.0936} & {0.0125}
& {0.2468} & {0.0449} 
& {0.1696} & {0.0269} \\
\cmidrule{2-14}
{} &{BERT4Rec} 
& {0.2311} & {0.0396} 
& {0.1348} & {0.0244} 
& {0.0771} & {0.0107} 
& {0.1077} & {0.0153}
& {0.2303} & {0.0411} 
& {0.1500} & {0.0225} \\
\cmidrule{2-14}
{} &{Comirec} 
& {0.2486} & {0.0426} 
& {0.1058} & {0.0207} 
& {0.0692} & {0.0096} 
& {0.1872} & {0.0273}
& {0.2163} & {0.0387} 
& {0.1576} & {0.0262} \\
\cmidrule{2-14}
{} &{SASRec} 
& {0.3144} & {0.0546} 
& {0.3029} & {0.0534} 
& {0.0719} & {0.0098} 
& {0.1538} & {0.0235}
& {0.3142} & {0.0524} 
& {0.1891} & {0.0306} \\
\cmidrule{2-14}
{Few-shot} &{PeterRec} 
& {0.2501} & {0.0440} 
& {0.2746} & {0.0500} 
& {0.0684} & {0.0094} 
& {0.2590} & {0.0382}
& {0.2735} & {0.0498} 
& {0.1957 } & {0.0311} \\
\cmidrule{2-14}
{Rec.} &{PAUP} 
& {0.2996} & {0.0516} 
& {0.2486} & {0.0455} 
& {0.0973} & {0.0144} 
& {0.1154} & {0.0170}
& {0.2506} & {0.0459} 
& {0.1679} & {0.0279} \\
\cmidrule{2-14}	
{} &{LightGCN} 
& {0.6221} & {0.1025} 
& {0.3609} & {0.0589} 
& {0.1253} & {0.0184} 
& {0.2526} & {0.0370}
& {0.4059} & {0.0684} 
& {0.2707} & {0.0428} \\
\cmidrule{2-14}
{} &{DisenGCN} 
& {0.5962} & {0.0869} 
& {0.4268} & {0.0716} 
& {0.0973} & {0.0138} 
& {0.2167} & {0.0313}
& {0.3359} & {0.0544} 
& {0.2022} & {0.0297} \\
\cmidrule{2-14}
{} &{SimGCL}
& {0.5057} & {0.0962} 
& {0.3167} & {0.0551} 
& {0.1113} & {0.0168} 
& {0.2244} & {0.0326}
& {0.4046} & {0.0676} 
& {0.1261} & {0.0198} \\
\cmidrule{2-14}
{} &{M2GNN} 
& {0.4818} & {0.0717} 
& {0.4594} & {0.0752} 
& {0.1218} & {0.0184} 
& {0.2846} & {0.0438}
& {0.3346} & {0.0558} 
& {0.2772} & {0.0422} \\
\cmidrule{2-14}
{} &{HIER} 
& {\textbf{0.6472}} & {\textbf{0.1062}} 
& {\textbf{0.5239}} & {\textbf{0.0848}} 
& {\textbf{0.1814}} & {\textbf{0.0286}} 
& {\textbf{0.4038}} & {\textbf{0.0615}}
& {\textbf{0.4377}} & {\textbf{0.0726}} 
& {\textbf{0.3641}} & {\textbf{0.0597}} \\
\cmidrule{1-14}
{Zero-shot} & {Tiger} 
& {0.1563} & {0.0374} 
& {0.3022} & {\textbf{0.0734}}  
& {\textbf{0.2840}} & {\textbf{0.0594}} 
& {0.2141} & {0.0474} 
& {0.2354} & {0.0484} 
& {0.3272} & {0.0903}  \\
\cmidrule{2-14}
{Rec.} &{HIER} 
& {\textbf{0.2934}} & {\textbf{0.0549}} 
& {\textbf{0.3109}} & {0.0626}  
& {0.2489} & {0.0492} 
& {\textbf{0.2833}} & {\textbf{0.0598}} 
& {\textbf{0.3626}} & {\textbf{0.0849}} 
& {\textbf{0.4663}} & {\textbf{0.1252}}  \\

\bottomrule
\end{tabular}}
\end{table*}
% \vspace{-1em}

